Meeting effectiveness and inclusiveness: large-scale measurement, identification of key features, and prediction in real-world remote meetings

Workplace meetings are vital to organizational collaboration, yet relatively little progress has been made toward measuring meeting effectiveness and inclusiveness at scale. The recent rise in remote and hybrid meetings represents an opportunity to do so via computer-mediated communication (CMC) systems. Here, we share the results of an effective and inclusive meetings survey embedded within a CMC system in a diverse set of companies and organizations. We correlate the survey results with objective metrics available from the CMC system to identify the generalizable attributes that characterize perceived effectiveness and inclusiveness in meetings. Additionally, we explore a predictive model of meeting effectiveness and inclusiveness based solely on objective meeting attributes. Lastly, we show challenges and discuss solutions around the subjective measurement of meeting experiences. To our knowledge, this is the largest data-driven study conducted after the pandemic peak to measure, understand, and predict effectiveness and inclusiveness in real-world meetings at an organizational scale.

==> boneyard.tex <==
%A word on correlation vs causation: statistical modeling can rarely claim any insights on casual relations unless there are well-crafted controlled experiments in place {<\color{cyan} need a ref here>}. Our recommendation for using the results from current publications or similar ones is to use them to detect "potential" casual relations and develop campaigns and experiments to test their true casual impact in a real workplace. If an attribute does not show any connection in this modeling step, it may have already saturated any impact or is guaranteed that does not have any statistical connection with EIM metrics and can be set to lower priorities when planning. 

%\begin{itemize}
%    \item + Generalized findings outside of MS
%    \item + Suggested new features with data which show improved AUC
%    \item - Bias issues and solutions
%\end{itemize}


% understand what biases existed; namely, rater bias, response bias and anonymity bias. Our results from the initial tests with a small number of beta users of the CMC system confirmed the existence of three key issues;
%\begin{itemize}
%    \item The low response rates observed were a direct effect of having a 2-page survey compared to a 1-page. 
%    \item Users were clicking the 5-star rating to avoid having to answer follow-up questions on the second page for anything less than a 5-star rating.
%    \item Users were providing inflated ratings due to concerns with their ratings being shared with other stakeholders in the organization (lack of rating anonymity).
%\end{itemize}
%To address these issues we began a series of A/B experiments to improve data quality and the fidelity of our usable results. 



\begin{comment}
\subsection{Generalized Meeting Inclusiveness and Effectiveness Attributes}\label{sec:EIMattributes}
\begin{comment}
Previous findings in \cite{cutler_meeting_2021}, showed that certain meeting attributes are more important than others when it comes to meeting effectiveness and inclusiveness. Specifically: 

\begin{itemize}
    \item Meeting joined in-person or remotely using the CMC system
    \item Participation (measured as ‘speaking more than once in the meeting’)
    \item The presence of meeting agenda
    \item Reliable Calling/Meeting experience if joined remotely (e.g., no call drops, video freeze, or one-way audio,)
    \item Using video when joining remotely
    \item High Audio/Video Quality if joined remotely (e.g., no echo, noise, or speech distortion)
    \item Sharing pre- and post-reading material
\end{itemize}

The data presented in \cite{cutler_meeting_2021} was collected via email survey before the pandemic and includes respondents who joined meetings in person as well as respondents who joined meetings remotely using a CMC system. It showed that meetings, where everyone joined remotely using a CMC system, are more effective and inclusive than in-person or hybrid meetings. We call this form of meeting an all-remote meeting. All-remote meetings became dominant through the pandemic, which is the time period for the current paper's data collection. The new survey is embedded in the CMC system  and does not include respondents who join the meeting without the CMC system. So it is only reflecting the experience of remote participants. Since the time period of the new survey overlaps with the COVID-19 pandemic, it is expected that all-remote meetings have been the dominant type of meetings. As described in \ref{sec:method}, the new survey was extended to multiple companies from different industries to provide more robust conclusions. 

In contrast to the main model developed in \cite{cutler_meeting_2021} where all model variables came from the survey itself, the current modeling relies on telemetry to generate input variables such as meeting duration.  Telemetry is referred to any information that is available to the CMC system and is collected alongside the ratings. This provides an opportunity to measure many attributes more accurately. For example, how many minutes an attendee was on the call and for how long she could see other participants' videos is most likely not accurately reported in a survey. The rest of this section describes how telemetry is used to generate the variables needed for this study.
\end{comment}

%The resulting insights are shared in Section \ref{sec:graph}.

%Lack of data on meeting type: patterns are likely strongly affected by meeting type (e.g., results around screen-sharing). 

%Remote meetings became a dominant part of work life over the past few years. However, relatively little progress has been made toward measuring and understanding meeting effectiveness and inclusiveness. %An Effective and Inclusive Meeting (EIM) survey and predictive model was developed in {\color{cyan}[anonymous]} based on large survey data collected from the employees of a multinational corporation as well as integration into a widely used Computer-mediated Communication (CMC) system. This paper contains the extension of this research to a more diverse set of companies and organizations.
%In this paper, we share the results of an in-client survey on Effective and Inclusive Meetings (EIM) by a diverse set of companies and organizations. 
%To our knowledge, this is the largest data-driven study conducted after the pandemic started to measure and understand meeting effectiveness and inclusiveness. We show the generalizable attributes that characterize perceived inclusiveness and effectiveness in meetings conducted via a computer-mediated communication (CMC) system. We also show the challenges and discuss solutions for subjective measurement of meeting effectiveness and inclusiveness. 

%To our knowledge, there are no previous studies of meeting effectiveness that include meeting inclusiveness, AV quality and reliability, remote/local participants, comfortableness in participating, or pre-meeting written communication. 

%Garg and Johari \cite{garg_designing_2019} show that surveys with verbal descriptions of the choices give a much lower skew than numeric or star-based surveys, and that positive-skewed verbal descriptions of the choices are less prone to rater inflation where the ratings tend to increase over time. 

%We build on and substantially advance the previously developed multivariate model of factors associated with meeting effectiveness and inclusiveness [13]. 

%   For the next experiment we expanded our total set of addressable CMC system users to prevent an overlap with users who had already seen previous iterations. For this new set, the team implemented a two-factor experiment design with one control group and four treatment groups. The two factors are the percent of meetings selected at random ("Trigger Rate") and the minimum amount of time that needed to lapse before a user would be shown the survey at the end of the meeting ("Cooldown rate"). 

   %\item a small-scale email-based experiment to compare surveys with and without an explicit message about preserving rater anonymity.  % would result in a statistically significant change in response rate (\% of people that provided a rating) and rating skew (\% of raters who provided 5-star ratings). Three survey variants were sent out to approximately 3000 CMC system users, on which there was an ~10\% response rate. Users in the control group were shown the same language as the original in-client survey. Users in the first test group had a specific call out in the survey instructions to let them know their responses would remain anonymous. Users in the third and final test group had a different survey title which included language to let them know their ratings would remain anonymous.

   %\item Highlighting rater anonymity resulted in a statistically significant lower skew, similar to the one-page survey outcome described above. Typical consumer-facing rating systems do not have to be as sensitive to rater anonymity, but organizations trying to gather feedback from employees should be aware of this distinction.
%\item Ensuring that meetings were truly selected at random was essential to ensure that responses remained useful. Surveying the same users, even within a sub-group, resulted in bias due to rater fatigue, thereby reducing the usefulness of the results. This also means over surveying users will not help the group conclude on any changes in policy made to improve meeting effectiveness.

%After completing our initial set of experiments, we wanted to expand the scope of our dataset to include external customers of the CMC system (i.e., the participating organizations). 
%Two weeks following an email-based survey, we rolled out the in-client survey to a small proportion of meetings that were selected at random. However, some global organizations limited which countries' users would be eligible to receive the survey based on local rules and regulations (e.g., European Work Councils, working hour rules, etc.). 

%This study's data consists of subjective ratings provided by users and meeting attributes that are computed based on automated meeting telemetry submissions by the CMC system. 

%Graphical model  are tools for modeling the conditional dependencies among multiple variables.  introduces an algorithm to fit a special case of graphical models for the EIM metrics. The current study uses the same algorithm (with slight modifications) to reduce the available features into a smaller set and to learn the hierarchy of these correlations with the main EIM outcome metrics: 1. Effective, 2. Inclusive, 3. Participation. The algorithm is aware of this hierarchy, but there is no other restriction in terms of the graph structure. 

%\begin{itemize}
%    \item Meetings where everyone participates are 1.8\% more Effective and 2.6\% more Inclusive.
%    \item Meetings with less than 50\% participation are 1.5\% less Effective and 2.7\% less inclusive.
%\end{itemize}

%We also found higher PMR EMR, IMR when there were more meetings on that day (get numbers).  We checked the number of meetings in a day with time to the next meeting to see if there was an interaction effect where time till the next meeting was more important for predicting EMR, PMR, IMR for people with a large number of meetings in a day, however, there was no statistically different change in these metric values.
% (~9.8 response rate for 2-3 meetings, and 7\% rr for 9+ meetings). 

%In the telemetry data, we store a user id which within our data doesn't identify the end user.  However, other data sources can be joined with this data that would identify the end user.  For this reason, we cannot include a statement that the data is anonymous.  

% Enabling Specification 2402018: Anonymization Experiment: compare baseline - Boards (visualstudio.com)  Email2: 82\%,  n=137, CI: (75\%, 88\%), EMF in the same time period as Email2: 97\%, n = ~2,000, Email1: 83\%, n=3,290.  (Was there any in client testing? - no)

%{\color{cyan} anything else on specific attributes, generalizability, or prediction?}

% {\color{cyan} interventions to improve meetings, challenges and concerns around privacy/surveillance}


%This result is consistent with previous studies based on user declared Participation as in \cite{cutler_meeting_2021-1}. A number of important features of a remote meeting is also understood via their correlation with Participation rather than subjective ratings directly.


%Given its high rank in the list of meeting attributes that correlate with effectiveness and inclusiveness, Participation is the most important variable that we analyze. Section \ref{sec:participation} contains the results of this analysis. 
%The rest of attributes are discussed in this section by zooming into different parts of the graph structure

%While ScreenShare is undoubtedly beneficial and necessary for some meetings and increases meeting effectiveness significantly, one should be aware that long screensharing in the call does have the side effect of reducing participation for all attendees.  

% This strong link has inspired the development of new features to enhance participation for remote attendees. An example of such features is introduced in {\color{cyan}ref to failed-speech-interruption paper}.

%Given the limited sample size for some organizations, it was impossible to have organization-specific graph models. Instead, we divided the participating companies into two different groups and compared their graphs. 

%\begin{figure}
% \centering
% \includegraphics[width=0.6\linewidth]{figs/auc_generalizability.png}
% \caption{AUC.}  
% \label{fig:auc}
%\end{figure}

%(PMR from 98\% to 84\% EMR 98-> 95\% IMR 98\%->95.  Avoiding actual rates as the baselines are different than above data...  Ask yasaman)


\begin{comment}
\vskip 0.1in
Along the way, there were several challenges we encountered:
\begin{enumerate}
    \item Survey respondents needed more clarity from both our and their organization about how responses would be used.
    \item Executives wanted a clear line of sight to our models' ability to show statistically significant changes based on any changes the organization made to improve meeting culture. 
    \item Our organization was concerned about how explainable the model would be for external stakeholders.
    \item Human Resources and IT stakeholders were not comfortable with sending mass emails (i.e., company-wide surveys). Alternatives like posting the survey to internal social channels %(i.e., Yammer) 
    resulted in a minimal response rate (less than 3 percent). This prevented our ability to collect a diverse baseline using this methodology.
\end{enumerate}    
\end{comment}

%Section \ref{sec:experiment} describes the details of the A/B experiments we conducted to increase the amount of usable data and resulting quality. 

    %\item subjective ratings of traditional surveys are prone to strong skew unless alternative wording is applied 

\begin{comment}
    \subsubsection{Pilot Program Learnings and Outcomes}\label{sec:pilot}
When we initially reached out to organizations that could be potentially interested in participating in the pilot program, the most requested feature in our post-pilot reports was the ability to slice the resulting data by the companies' organizational structure (e.g.line of business, team size and others). Unfortunately, like this request, there were many features we could not commit time and development effort to; therefore, it is important to manage stakeholder expectations, especially when running experiments with external customers. Furthermore, below are a few more things we would incorporate were we to run the same or similar program in the future;
\begin{enumerate}
    \item Getting executives to agree to support a pilot program is step one, but step 2 is to mitigate end-user concerns with collecting sensitive data, like meeting ratings. Unfortunately, we were forced to turn off the in-client survey for one of the participating customers due to employee concerns. In the future, it is crucial to over-communicate and collaborate with stakeholders to build a central set of resources that end-users can refer to if they have questions. 
    \item While executives focused on business outcomes will be supportive of new programs like this pilot, unwritten rules like culture, diversity, and inclusion priorities, and HR/Legal teams will have concerns that need to be addressed. Therefore, it is essential to uncover and address these concerns as early as possible to ensure the pilot will be feasible for the customer.
    \item  Customers of our software are local and global companies. For global companies, it is essential to have a robust deployment system that can be configured to fit various business requirements. Examples of requirements include; only certain users from certain countries should be eligible to receive the survey, varying the random meeting selection rate, and selecting only a subset of the organization 
\end{enumerate}

Ultimately, when rolling out experiments to external organizations has social, cultural, and technical challenges. To ensure project success the team should be aware that while buy-in from executive stakeholders is a positive sign, it's not enough until human resources, information technology, and end-users have a thorough understanding of the objectives. Project owners should try to brainstorm potential blockers and provide guidance, written or verbal, proactively to any relevant stakeholders. 

\end{comment}

\begin{comment}

\begin{table}
\begin{tabularx}{0.7\textwidth}{
l >{\raggedright\arraybackslash}X
l >{\centering\arraybackslash}X
l >{\centering\arraybackslash}X 
l >{\centering\arraybackslash}X }
\hline
Participation Bins & Effective Rate (error) & Inclusive Rate (error) & Number of Meetings\\
\hline
100\% & 0.99 (0.0) & 0.99 (0.0) & 1820\\
\hline
40\% - 99\% & 0.98 (0.0) & 0.98 (0.0) & 2043\\
\hline
LessThan40\% & 0.97 (0.0) & 0.96 (0.0) & 3551\\
\hline
\end{tabularx}
\caption{\label{tab:Participation}Per-meeting Effective and Inclusive raters by different levels of meeting-level Participation. Error bounds that are in parenthesis are 95\% Confidence Interval bounds for the meeting level ratings.}
\end{table}
\end{comment}
